Accelerating material melting temperature predictions by implementing machine learning potentials in the SLUSCHI package

The SLUSCHI (Solid and Liquid in Ultra Small Coexistence with Hovering Interfaces) automated package, with interface to the first-principles code VASP (Vienna Ab initio Simulation Package), was developed by us for efficiently determining the melting temperatures of various materials. However, performing many molecular dynamics simulations for small liquid-solid coexisting supercells to predict the melting temperature of a material is still computationally expensive, often requiring weeks and tens to hundreds of thousands of CPU hours to complete. In the present paper, we made an attempt to interface the SLUSCHI package with the highly efficient molecular dynamics LAMMPS code and demonstrated that it achieves a much faster melting temperature determination, outperforming the original VASP-based approach by at least one order of magnitude. In our melting temperature calculations, the LAMMPS simulations were performed based on the LASP (Large-scale Atomic Simulation) machine learning potentials which are pre-built using first-principles data. Besides the dramatic CPU time reduction for melting temperature predictions the calculated melting temperatures for various materials (simple and transition metals, alloys, oxides and carbide) are reasonably accurate. Analysis of the calculated results shows that 60% of the melting temperatures are within 200 K of experimental values with the RMSE value of 187 K which is slightly worse than the first-principles DFT RMSE value of 151 K. Therefore, interfacing SLUSCHI with LAMMPS molecular dynamics simulations makes it possible to quickly screen out the best candidates from numerous materials in a much more efficient way, and facilitate the rational design of materials within the framework of the materials genome paradigm.

==> iron_melting_curve/Tables/LASP_ML_corrected_Experimental_data_old.tex <==
%\documentclass{article}
%\usepackage{booktabs}

%\begin{document}

\begin{center}
\begin{table}
    \centering
    \caption{Material System Comparison}
    \label{tab:corrected_single}
    \begin{tabular}{l|r|r|r|l}
    \hline
    Material & $T_m^\mathrm{ML}$ &  Corrected $T_m^\mathrm{DFT}$ & $T_m^\mathrm{exp.}$ & ML Potential \\
    \hline
    Pd & $1830 \pm 5$ & 1850 & 1810 & PdAgTiOH \\
    Ag & $1326 \pm 19$ & 1302 & 1208 & PdAgTiOH \\
    Ti & $1650 \pm 14$ & 1934 & 1957 & PdAgTiOH\\
    Ti & $1801 \pm 19$ & 1912 & 1957 & TiOH\\
    Mo & $2656 \pm 23$ & 2780 & 2782 & PtNiMoOH\\
    Pt & $1805 \pm 5$ & 1930 & 2090 & PtNiMoOH\\
    Ni & $1703 \pm 7$ & 1735 & 1752 & PtNiMoOH\\
    Pd & $1811 \pm 22$ & 1784 & 1810 & PdNiCHO\\
    Ni & $1709 \pm 6$ & - & 1752 & PdNiCHO\\
    Pt & $1863 \pm 9$ & - & 2090 & PtSnSiO\\
    Mg & $1193 \pm 13$ & - & 923 & AlMgTi\\
    Al & $1170 \pm 11$ & - & 1040 & AlMgTi\\
    Zr & $1950 \pm 18$ & 2403 & 2114 & ZrOH\\
    Zr & $1948 \pm 26$ & 2327 & 2114 & ZrOH\\ %smaller unit cell size
    Fe BCC & $1940 \pm 6$ & - & 1811 & FeCr\\
    Fe BCC & $1774 \pm 17$ & - & 1811 & FeCr\\ %smaller unit cell size
    Fe FCC & $1721 \pm 55$ & - & 1811 & FeCr\\
    W & $3613 \pm 19$ & 3386 & 3695 & WCH\\
    Cu & $1050 \pm 31$ & - & 1358 & PdCuAg\\
    Cu & $1130 \pm 5$ & - & 1358 & CuAlOH\\
    \hline
    RMSE & 181 & 150 & \\
    \bottomrule
    \end{tabular}
\end{table}
\end{center}

%\end{document}


==> iron_melting_curve/Tables/LASP_ML_experimental_data.tex <==
\begin{table}
    \centering
    \caption{Comparison of melting temperatures calculated from \texttt{LASP} ML potentials}
    \label{tab:single_component}
    \begin{tabular}{l|r|r|r|r|l}
    \hline
     Material &  $T_m^\mathrm{ML}$ &  $T_m^\mathrm{Corrected}$ & $T_m^\mathrm{VASP}$ & $T_m^\mathrm{exp}$ & ML Potential \\
    \hline
    Ag & $1326 \pm 19$ & 1302 & - & 1208 & PdAgTiOH \\    
    Al & $1170 \pm 11$ & - & 1040 & 933 &  AlMgTi\\
    Cu & $1050 \pm 31$ & - & - & 1358 & PdCuAg\\ %smaller unit cell size
    Cu & $1130 \pm 5$ & - & - & 1358 &  CuAlOH\\\
    Fe & $1774 \pm 17$ & - & - & 1811 & FeCr\\
    Mg & $1186 \pm 13$ & - & - & 923 &  AlMgTi\\
    Mo & $2656 \pm 23$ & 2780 & - & 2782 & PtNiMoOH \\
    Ni & $1703 \pm 7$ & 1745 & - & 1752 &  PtNiMoOH\\
    Ni & $1709 \pm 6$ & - & - & 1752 & PdNiCHO \\
    Pd & $1830 \pm 5$ & 1850 & - & 1810 &  PdAgTiOH  \\
    Pd & $1811 \pm 22$ & 1784 & - & 1810 &  PdNiCHO\\
    Pt & $1805 \pm 5$ & 1930 & - & 2090 &  PtNiMoOH\\
    Pt & $1863 \pm 9$ & - & - & 2090 &  PtSnSiO\\ 
    Ti  & $1650 \pm 14$ & 1934 & 1750 & 1957 &  PdAgTiOH \\
    Ti  & $1801 \pm 19$ & 1912 & 1750 & 1957 &  TiOH \\
    W & $3613 \pm 19$ & - & 3497 & 3695 & WCH\\
    Zr & $1950 \pm 18$ & 2403 & 2114 & 2128 & ZrOH\\
     \hline
    RMSE & 188 & 113 & 151 \\
    \bottomrule
    \end{tabular}
\end{table}

==> iron_melting_curve/Tables/LASP_ML_experimental_data_old.tex <==
%\documentclass{article}
%\usepackage{booktabs}

%\begin{document}

\begin{table}
    \centering
    \caption{Comparison of melting temperatures calculated from \texttt{LASP} ML potentials}
    \label{tab:single_component}
    \begin{tabular}{l|r|r|r|l}
    \hline
     Material &  $T_m^\mathrm{ML}$ &  $T_m^\mathrm{exp}$ & $T_m^\mathrm{VASP}$ & ML Potential \\
    \hline
    Pd & $1830 \pm 5$ &\hspace{1.cm} 1810 & - & PdAgTiOH  \\
    Ag & $1326 \pm 19$ & 1208 & - & PdAgTiOH \\
    Ti  & $1650 \pm 14$ & 1957 & 1750 & PdAgTiOH \\
    Ti  & $1801 \pm 19$ & 1957 & 1750 & TiOH \\
    Mo & $2656 \pm 23$ & 2782 & - & PtNiMoOH \\
    Pt & $1805 \pm 5$ & 2090 & - & PtNiMoOH\\
    Ni & $1703 \pm 7$ & 1752 & - & PtNiMoOH\\
    Pd & $1811 \pm 22$ & 1810 & - & PdNiCHO\\
    Ni & $1709 \pm 6$ & 1752 & - & PdNiCHO \\
    Pt & $1863 \pm 9$ & 2090 & - & PtSnSiO\\ 
    Mg & $1193 \pm 13$ & 923 & 903 & AlMgTi\\
    Al & $1170 \pm 11$ & 933 & 1040 & AlMgTi\\
    Zr & $1950 \pm 18$ & 2128 & 2114 & ZrOH\\
    Zr & $1948 \pm 26$ & 2128 & 2114 & ZrOH\\ %smaller unit cell size
    Fe BCC & $1940 \pm 6$ & 1811 & - & FeCr\\ 
    Fe BCC & $1774 \pm 17$ & 1811 & - & FeCr\\ %smaller unit cell size
    Fe FCC & $1721 \pm 55$ & 1811 & - &FeCr\\ %smaller unit cell size
    W & $3613 \pm 19$ & 3695 & 3497 & WCH\\
    Cu & $1050 \pm 31$ & 1358 & - & PdCuAg\\ %smaller unit cell size
    Cu & $1130 \pm 5$ & 1358 & - & CuAlOH\\\hline %smaller unit cell size
     \hline
    RMSE & 181 & & \\
    \bottomrule
    \end{tabular}
\end{table}

%\end{document}
%\hspace{1.cm} will set the spacing in the columns
%Zr HCP & $1417 \pm 13$ & 2114 & ZrOH\\
%W HCP & $0 \pm 0$ & 3695 & WCH\\

==> iron_melting_curve/Tables/LASP_compound_corrected.tex <==
%\documentclass{article}
%\usepackage{booktabs}

%\begin{document}

\begin{table}
    \centering
    \caption{Compound Data Comparison with Data Correction}
    \label{tab:compound_correction}
    \begin{tabular}{l|r|r|r|l}
    \hline
    Material & $T_m^\mathrm{ML} $ & Corrected $T_m^\mathrm{DFT}$ & $T_m^\mathrm{exp}$ & ML Potential \\
    \hline
    AgPd & $1875 \pm 19$ & 1913 & 1566 & PdAgTiOH \\
    Fe$_2$O$_3$ & $1649 \pm 13$ & 1574 & 1856 & FeOH \\
    Fe$_3$O$_4$ & $1718 \pm 5$ & - & 1867 & FeOH \\
    FeO & $1750 \pm 13$ & - & 1633 & FeOH \\
    HfO$_2$ & $2986 \pm 29$ & - & 3031 & SiHfOH \\
    Ni$_{0.9}$Mo$_{0.1}$ & $1842 \pm 13$ & 1914 & 1728 & PtNiMoOH \\
    NiO & $2509 \pm 9$ & - & 2228 & NiO\\ 
    TiAl$_3$ & $1933 \pm 15$ & - & 1673 & AlMgTi \\
    TiO$_2$ & $1969 \pm 6$ & 2063 & 2093 & TiOH \\
    WC & $3204 \pm 12$ & - & 3145 & WCH \\
    Y$_2$O$_3$ &  $2790 \pm 27$ & - & 2718 & PtYO \\
    ZrO$_2$ & $3013 \pm 35$ & - & 2988 & ZrOH \\
    ZrO$_2$ & $2685 \pm 61$ & - & 2988 & ZrO \\
    \hline
    RMSE & 159 & 246 & \\
    \bottomrule
    \end{tabular}
\end{table}

%\end{document}
% TiO$_2$ & $1969 \pm 6$ & 2063 & 2093 & TiOH \\
%    AgPd & $1875 \pm 19$ & 1913 & 1566 & PdAgTiOH \\
 %   Ni$_{0.9}$Mo$_{0.1}$ & $1842 \pm 13$ & 1914 & 1728 & PtNiMoOH \\
  %  TiAl$_3$ & $1933 \pm 15$ & - & 1673 & AlMgTi \\
  %  FeO & $1750 \pm 13$ & - & 1633 & FeOH \\
  %  Fe$_2$O$_3$ & $1649 \pm 13$ & 1574 & 1856 & FeOH \\
  %  Fe$_3$O$_4$ & $1718 \pm 5$ & - & 1867 & FeOH \\
  %  WC & $3285 \pm 105$ & - & 3145 & WCH \\
  %  WC & $3204 \pm 12$ & - & 3145 & WCH \\ %smaller unit cell
  %  HfO$_2$ & $2986 \pm 29$ & - & 3031 & SiHfOH \\
   % SiC & $0 \pm 0$ & 0 & - & SiAlPHON \\
  %  ZrO$_2$ & $3013 \pm 35$ & - & 2988 & ZrOH \\
  %  ZrO$_2$ & $2685 \pm 61$ & - & 2988 & ZrO \\
  %  TiO$_2$ & $2062 \pm 77$ & - & 2093 & TiOH \\

==> iron_melting_curve/Tables/LASP_compound_old.tex <==
\begin{table}
    \centering
    \caption{Compound Data Comparison}
    \label{tab:compound_uncorrection}
    \begin{tabular}{l|r|r|l}
    \hline
    Material & $T_m^\mathrm{ML} $ & $T_m^\mathrm{exp}$ &  ML Potential \\
    \hline
    TiO$_2$ & $1969 \pm 6$ & 2093 & TiOH \\
    AgPd & $1875 \pm 19$  & 1566 & PdAgTiOH \\
    Ni$_{0.9}$Mo$_{0.1}$ & $1842 \pm 13$ &  1728 & PtNiMoOH \\
    TiAl$_3$ & $1933 \pm 15$ &  1673 & AlMgTi \\
    FeO & $1750 \pm 13$ & 1633 & FeOH \\
    Fe$_2$O$_3$ & $1649 \pm 13$ & 1856 & FeOH \\
    Fe$_3$O$_4$ & $1718 \pm 5$ &  1867 & FeOH \\
    WC & $3285 \pm 105$ & 3145 & WCH \\
    WC & $3204 \pm 12$ & 3145 & WCH \\ %smaller unit cell
    HfO$_2$ & $2986 \pm 29$ & 3031 & SiHfOH \\
    %SiC & $0 \pm 0$ & 0 & - & SiAlPHON \\
    ZrO$_2$ & $3013 \pm 35$ & 2988 & ZrOH \\
    ZrO$_2$ & $2685 \pm 61$ & 2988 & ZrO \\
    TiO$_2$ & $2062 \pm 77$ & 2093 & TiOH \\
    \hline
    RMSE & 159 & & \\
    \bottomrule
    \end{tabular}
\end{table}

==> iron_melting_curve/Tables/Total_lasp_results.tex <==
\begin{table}
    \centering
    \caption{Comparison of melting temperatures calculated from \texttt{LASP} ML potentials}
    \label{tab:total_lasp}
    \begin{tabular}{l|r|r|r|r|l}
    \hline
     Elements &  $T_m^\mathrm{ML}$ &  $T_m^\mathrm{Corrected}$ & $T_m^\mathrm{VASP}$ & $T_m^\mathrm{exp}$ & ML Potential \\
    \hline
    Ag & $1326 \pm 19$ & 1302 & - & 1208 & PdAgTiOH \\    
    Al & $1170 \pm 11$ & - & 1040 & 933 &  AlMgTi\\
    Cu & $1050 \pm 31$ & - & - & 1358 & PdCuAg\\ %smaller unit cell size
    Cu & $1130 \pm 5$ & - & - & 1358 &  CuAlOH\\\
    Fe & $1774 \pm 17$ & - & - & 1811 & FeCr\\
    Mg & $1186 \pm 13$ & - & - & 923 &  AlMgTi\\
    Mo & $2656 \pm 23$ & 2780 & - & 2782 & PtNiMoOH \\
    Ni & $1703 \pm 7$ & 1745 & - & 1752 &  PtNiMoOH\\
    Ni & $1709 \pm 6$ & - & - & 1752 & PdNiCHO \\
    Pd & $1830 \pm 5$ & 1850 & - & 1810 &  PdAgTiOH  \\
    Pd & $1811 \pm 22$ & 1784 & - & 1810 &  PdNiCHO\\
    Pt & $1805 \pm 5$ & 1930 & - & 2090 &  PtNiMoOH\\
    Pt & $1863 \pm 9$ & - & - & 2090 &  PtSnSiO\\ 
    Ti  & $1650 \pm 14$ & 1934 & 1750 & 1957 &  PdAgTiOH \\
    Ti  & $1801 \pm 19$ & 1912 & 1750 & 1957 &  TiOH \\
    W & $3613 \pm 19$ & - & 3497 & 3695 & WCH\\
    Zr & $1950 \pm 18$ & 2403 & 2114 & 2128 & ZrOH\\
     \hline
    RMSE & 188 & 113 & 151 \\
    \hline
    Compounds \\
    \hline
    AgPd & $1875 \pm 19$ & 1913 & - & 1566 & PdAgTiOH \\
    Fe$_2$O$_3$ & $1649 \pm 13$ & 1574 & - & 1856 & FeOH \\
    Fe$_3$O$_4$ & $1718 \pm 5$ & - & - & 1867 & FeOH \\
    FeO & $1750 \pm 13$ & - & - & 1633 & FeOH \\
    HfO$_2$ & $2986 \pm 29$ & - & - & 3031 & SiHfOH \\
    Ni$_{0.9}$Mo$_{0.1}$ & $1842 \pm 13$ & 1914 & - & 1728 & PtNiMoOH \\
    NiO & $2509 \pm 9$ & - & - & 2228 & NiO\\ 
    TiAl$_3$ & $1933 \pm 15$ & - & - & 1673 & AlMgTi \\
    TiO$_2$ & $1969 \pm 6$ & 2063 & - & 2093 & TiOH \\
    WC & $3204 \pm 12$ & - & - & 3145 & WCH \\
    Y$_2$O$_3$ &  $2790 \pm 27$ & - & - & 2718 & PtYO \\
    ZrO$_2$ & $3013 \pm 35$ & - & - & 2988 & ZrOH \\
    ZrO$_2$ & $2685 \pm 61$ & - & - & 2988 & ZrO \\
    \hline
    RMSE & 159 & 246  \\
    \hline
    Total RMSE & 174 & 179 \\
    \bottomrule
    \end{tabular}
\end{table}

==> iron_melting_curve/Tables/old/VASP_ML_DFT_Experimental.tex <==
%\documentclass{article}
%\usepackage{booktabs}

%\begin{document}

\begin{table}[htbp]
    \centering
    \caption{ML, DFT, and experimental melting temperatures \cite{SLUSCHI_table_1,SLUSCHI_table_2,SLUSCHI_table_3,SLUSCHI_table_4}}
    %\caption{Material System Comparison}
    \label{tab:material_system_comparison}
    \begin{tabular}{l|r|r|r}
    \hline
    Material & $T_m^\mathrm{ML}$ [K] & $T_m^\mathrm{DFT}$ [K]& $T_m^\mathrm{exp}$ [K] \\
    \midrule
    \hline
    Mg & \hspace{.99cm}$861 \pm 41$ & \hspace{.99cm} $903 \pm 40$ & \hspace{1.5cm} 923 \\
    %\hline
    Al & $1062 \pm 72$ & $1040 \pm 13$ & 933 \\
    %\hline
    Ta & $3084 \pm 92$ & $3194 \pm 40$ & 3293 \\
    %\hline
    Ti & $1590 \pm 28$ & $1952 \pm 45$ & 1941 \\
    %\hline
    Ti & $1869 \pm 71$ & $1952 \pm 45$ & 1941 \\
    %\hline
    W & $3816 \pm 92$ & $3470 \pm 45$ & 3695 \\
    %\hline
    W* & $3556 \pm 29$ & $3470 \pm 45$ & 3695 \\
    %\hline
    Zr{\color{red}**} & $1787 \pm 29$ & $2114 \pm 30$ & 2128 \\
    %\hline
    Zr & $1934 \pm 94$ & $2114 \pm 30$ & 2128 \\
    \hline
    RMSE & 217 & 124 & \\
    \end{tabular}
\end{table}

%\end{document}


==> iron_melting_curve/Tables/old/VASP_data_table.tex <==
%\documentclass{article}
%\usepackage{multirow}
%\usepackage{rotating}

%\begin{document}

\begin{table*}[htbp]
    \centering
    %\caption{System Characteristics}
    %\label{tab:system_characteristics}
    \caption{This table contains the results for all the VASP simulations run in this study and the data from systems run using SLUSCHI and standard DFT VASP. \cite{SLUSCHI_table_1,SLUSCHI_table_2,SLUSCHI_table_3,SLUSCHI_table_4} The data contained within the table includes the name of the system being tested, the melting temperature calculated with either the ML protocols used for this study or with standard DFT VASP. The radius of the simulation cell in Angstroms, the total number of atoms within the simulation, the total number of MD trajectories run within the simulation, the total number of CPU hours each simulation, and the total number of days a simulation took.}
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    \hline
    \multirow{2}{*}{System} & \multirow{2}{*}{$T_m^\mathrm{ML}$ (K)} & \multirow{2}{*}{$T_m^\mathrm{DFT}$ (K)} & \multirow{2}{*}{Radius(\AA)} & \multirow{2}{*}{Atoms In Simulation} & \multirow{2}{*}{MD Trajectories} & \multirow{2}{*}{CPU hours} & \multirow{2}{*}{Days} \\
    & & & & & & & \\
    \hline
    Mg & 861 $\pm$ 41 & - & 10.4 & 96 & 27 & 12,421 & 59 \\
    \hline
    Mg & - & 903 $\pm$ 40 & 9.4 & 72 & 29 & 304 & 2 \\
    \hline
    Al & 1062 $\pm$ 77 & - & 9.9 & 128 & 17 & 5,694 & 45 \\
    \hline
    Al & - & 919 $\pm$ 6 & 10.3 & 120 & 30 & 2,478 & 2 \\
    \hline
    Ta & 3084 $\pm$ 92 & - & 9.4 & 96 & 26 & 23,530 & 53 \\
    \hline
    Ta & - & 3194 $\pm$ 40 & 10 & - & 38 & 54,000 & 24 \\
    \hline
    Ti & 1590 $\pm$ 28 & - & 9.8 & 112 & 55 & 122,380 & 124 \\
    \hline
    Ti & 1869 $\pm$ 71 & - & 10.8 & 128 & 30 & 75,543 & 20 \\
    \hline
    Ti & - & 1952 $\pm$ 45 & 10 & - & 48 & 20,000 & 20 \\
    \hline
    W & 3816 $\pm$ 92 & - & 9.6 & 96 & 25 & 13,332 & 32 \\
    \hline
    W & 3556 $\pm$ 29 & - & 10.5 & 128 & 38 & 139,684 & 124 \\
    \hline
    W & - & 3470 $\pm$ 45 & 10 & - & 30 & 38,500 & 18 \\
    \hline
    Zr & 1787 $\pm$ 29 & - & 10.1 & 88 & 30 & 74,311 & 114 \\
    \hline
    Zr & 1934 $\pm$ 94 & - & 10.7 & 96 & 21 & 30,842 & 9 \\
    \hline
    Zr & - & 2114 $\pm$ 30 & 9.7 & 96 & 27 & 17,841 & 24 \\
    \hline
    \end{tabular}
    \label{tab:system_characteristics}
\end{table*}

%\end{document}


==> lw/Tables/CPU_time.tex <==
\begin{table}
    \centering
    \caption{Computational details for the LASP simulations, including: Radius of the simulation cell and, number of atoms in the simulation. As well as a the CPU times for melting temperature prediction with the LASP method, and the DFT method.(For the Ti samples the different values for the DFT CPU column come different simulations. (*) one with the best melting temperature and (**) one with the best simulation time.  }
    \label{tab:total_lasp}
    \begin{tabular}{lcrccl}
    \hline
     Systems &   Radius (\AA) & N  & LASP & DFT   & LASP   \\
        & & & CPU Hours & CPU Hours & Potential \\    
    \hline
    Ag & 17 & 512 & 1,205 & - & PdAgTiOH \\    
    Al & 16 & 512 & 645 & 5,400 &  AlMgTi\\
    Cu & 10 & 192 & 3,643 & - & PdCuAg\\ %smaller unit cell size
    Cu & 10 & 192 & 5,458 & - &  CuAlOH\\\
    Fe & 10 & 208 & 1,606 & - & FeCr\\
    Mg & 16 & 360 & 679 & 304 &  AlMgTi\\
    Mo & 16 & 500 & 423 & - & PtNiMoOH \\
    Ni & 16 & 800 & 992 & - &  PtNiMoOH\\
    Ni & 16 & 800 & 582 & - & PdNiCHO \\
    Pd & 16 & 512 & 919 & - &  PdAgTiOH  \\
    Pd & 16 & 512 & 459 & - &  PdNiCHO\\
    Pt & 16 & 512 & 230 & - &  PtNiMoOH\\
    Pt & 16 & 512 & 435 & - &  PtSnSiO\\ 
    Ti & 16 & 500 & 697 & 20,000* &  PdAgTiOH \\ % best temperature
    Ti & 16 & 500 & 694 & 7,900** &  TiOH \\ % best time
    W & 10 & 132 & 869 & 35,900 & WCH\\
    Zr & 15 & 336 & 402 & 17,841 & ZrOH\\
%     \hline
%    RMSE & 188 & 113 & 151 \\
%    \hline
%    Compounds \\
%    \hline
    AgPd & 16 & 408 & 1,636 & - & PdAgTiOH \\
    Fe$_2$O$_3$ & 16 & 960 & 812 & - & FeOH \\
    Fe$_3$O$_4$ & 16 & 896 & 1,628 & - & FeOH \\
    FeO & 16 & 1,024 & 1,016 & - & FeOH \\
    HfO$_2$ & 15 & 648 & 1,588 & 7,900 & SiHfOH \\
    Ni$_{0.9}$Mo$_{0.1}$ & 14 & 576 & 532 & - & PtNiMoOH \\
    NiO & 16 & 928 & 1,034 & - & NiO\\ 
    TiAl$_3$ & 15 & 512 & 1,391 & - & AlMgTi \\
    TiO$_2$ & 17 & 780 & 3,122 & - & TiOH \\
    WC & 15 & 696 & 909 & - & WCH \\
    Y$_2$O$_3$ & 16 & 600 & 1,380 & - & PtYO \\
    ZrO$_2$ & 10 & 192 & 1,703 & - & ZrOH \\
    ZrO$_2$ & 10 & 192 & 1,558 & - & ZrO \\
%    \hline
%    RMSE & 159 & 246  \\
    \hline
%    Total RMSE & 174 & 179 \\
    \bottomrule
    \end{tabular}
\end{table}

==> lw/Tables/Total_lasp_results1.tex <==
\begin{table}
    \centering
    \caption{Comparison of melting temperatures calculated from \texttt{LASP} machine learning potentials with the \texttt{VASP} and experimental values. The \texttt{VASP} results were reported in Ref. xxx and the experimental values from Ref. xxx. All temperatures are in K. }
    \label{tab:total_lasp}
    \begin{tabular}{lrrrrl}
    \hline
     Systems &  $T_m^\mathrm{ML}$ &  $T_m^\mathrm{Corrected}$ & $T_m^\mathrm{VASP}$  & $T_m^\mathrm{exp}$ & ML Potential \\
    \hline
    Ag & $1326 \pm 19$ & 1302 & - & 1208 & PdAgTiOH \\    
    Al & $1170 \pm 11$ & - & 1040 & 933 &  AlMgTi\\
    Cu & $1050 \pm 31$ & - & - & 1358 & PdCuAg\\ %smaller unit cell size
    Cu & $1130 \pm 5$ & - & - & 1358 &  CuAlOH\\\
    Fe & $1774 \pm 17$ & - & - & 1811 & FeCr\\
    Mg & $1186 \pm 13$ & - & - & 923 &  AlMgTi\\
    Mo & $2656 \pm 23$ & 2780 & - & 2782 & PtNiMoOH \\
    Ni & $1703 \pm 7$ & 1745 & - & 1752 &  PtNiMoOH\\
    Ni & $1709 \pm 6$ & - & - & 1752 & PdNiCHO \\
    Pd & $1830 \pm 5$ & 1850 & - & 1810 &  PdAgTiOH  \\
    Pd & $1811 \pm 22$ & 1784 & - & 1810 &  PdNiCHO\\
    Pt & $1805 \pm 5$ & 1930 & - & 2090 &  PtNiMoOH\\
    Pt & $1863 \pm 9$ & - & - & 2090 &  PtSnSiO\\ 
    Ti  & $1650 \pm 14$ & 1934 & 1750 & 1957 &  PdAgTiOH \\
    Ti  & $1801 \pm 19$ & 1912 & 1750 & 1957 &  TiOH \\
    W & $3613 \pm 19$ & - & 3497 & 3695 & WCH\\
    Zr & $1950 \pm 18$ & 2403 & 2114 & 2128 & ZrOH\\
%     \hline
%    RMSE & 188 & 113 & 151 \\
%    \hline
%    Compounds \\
    \hline
    AgPd & $1875 \pm 19$ & 1913 & - & 1566 & PdAgTiOH \\
    Fe$_2$O$_3$ & $1649 \pm 13$ & 1574 & - & 1856 & FeOH \\
    Fe$_3$O$_4$ & $1718 \pm 5$ & - & - & 1867 & FeOH \\
    FeO & $1750 \pm 13$ & - & - & 1633 & FeOH \\
    HfO$_2$ & $2986 \pm 29$ & - & - & 3031 & SiHfOH \\
    Ni$_{0.9}$Mo$_{0.1}$ & $1842 \pm 13$ & 1914 & - & 1728 & PtNiMoOH \\
    NiO & $2509 \pm 9$ & - & - & 2228 & NiO\\ 
    TiAl$_3$ & $1933 \pm 15$ & - & - & 1673 & AlMgTi \\
    TiO$_2$ & $1969 \pm 6$ & 2063 & - & 2093 & TiOH \\
    WC & $3204 \pm 12$ & - & - & 3145 & WCH \\
    Y$_2$O$_3$ &  $2790 \pm 27$ & - & - & 2718 & PtYO \\
    ZrO$_2$ & $3013 \pm 35$ & - & - & 2988 & ZrOH \\
    ZrO$_2$ & $2685 \pm 61$ & - & - & 2988 & ZrO \\
%    \hline
%    RMSE & 159 & 246  \\
    \hline
    RMSE & 174 & 179 & 151 \\
    \hline
    \bottomrule
    \end{tabular}
\end{table}
